A Type-Directed, Dictionary-Passing Translation of Method Overloading and Structural Subtyping in Featherweight Generic Go

Featherweight Generic Go (FGG) is a minimal core calculus modeling the essential features of the programming language Go. It includes support for overloaded methods, interface types, structural subtyping and generics. The most straightforward semantic description of the dynamic behavior of FGG programs is to resolve method calls based on runtime type information of the receiver. This article shows a different approach by defining a type-directed translation from FGG- to an untyped lambda-calculus. FGG- includes all features of FGG but type assertions. The translation of an FGG- program provides evidence for the availability of methods as additional dictionary parameters, similar to the dictionary-passing approach known from Haskell type classes. Then, method calls can be resolved by a simple lookup of the method definition in the dictionary. Every program in the image of the translation has the same dynamic semantics as its source FGG- program. The proof of this result is based on a syntactic, step-indexed logical relation. The step-index ensures a well-founded definition of the relation in the presence of recursive interface types and recursive methods. Although being non-deterministic, the translation is coherent.

==> abbrevs.tex <==
\Cref{f:abbrev} defines some short-hand notations.

\boxfig{f:abbrev}{Abbreviations}{
  \begin{mathpar}
    \arraycolsep=14pt\def\arraystretch{1.6}
    \begin{array}{ll}
      \textrm{Abbreviation}              & \textrm{Full form}\\\hline
      \reduce{e}{e'}        & \reduceFG{\Multi{D}}{e}{e'}\\
      \reduce{\expT}{\expT'}        & \reduceTL{\tlMethTable}{\expT}{\expT'}\\
      \tdTypeTrans{}{\fgType}{V} & \tdTypeTrans{\fgEmptyEnv}{\fgType}{V} \\
      \tdTypeStarTrans{}{\fgType}{V} & \tdTypeStarTrans{\fgEmptyEnv}{\fgType}{V} \\
      \fgSub{}{\fgType}{\fgTypeAux} & \fgSub{\Multi{D}}{\fgType}{\fgTypeAux} \\
      \tdICons{}{\fgType}{\fgTypeAux}{V} & \tdICons{\pair{\Multi{D}}{\fgEmptyEnv}}{\fgType}{\fgTypeAux}{V} \\
      \tdICons{\fgTyEnv}{\fgType}{\fgTypeAux}{V} & \tdICons{\pair{\Multi{D}}{\fgTyEnv}}{\fgType}{\fgTypeAux}{V} \\
      \tdIDestr{}{\fgType}{\fgTypeAux}{V} & \tdIDestr{\pair{\Multi{D}}{\fgEmptyEnv}}{\fgType}{\fgTypeAux}{V} \\
      \tdIDestr{\fgTyEnv}{\fgType}{\fgTypeAux}{V} & \tdIDestr{\pair{\Multi{D}}{\fgTyEnv}}{\fgType}{\fgTypeAux}{V} \\
      \tdCheckSubst{}{\fgTyFormals}{\fgTyActuals}{\fgTySubst}{V} &
        \tdCheckSubst{\pair{\fgDecls}{\fgEmptyEnv}}{\fgTyFormals}{\fgTyActuals}{\fgTySubst}{V} \\
      \tdCheckSubst{\fgTyEnv}{\fgTyFormals}{\fgTyActuals}{\fgTySubst}{V} &
        \tdCheckSubst{\pair{\fgDecls}{\fgTyEnv}}{\fgTyFormals}{\fgTyActuals}{\fgTySubst}{V} \\
      \tdExpTrans{}{e : \fgType}{\expT}  & \tdExpTrans{\triple{\Multi{D}}{\fgEmptyEnv}{\fgEmptyEnv}}{e : \fgType}{\expT} \\
      \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e : \fgType}{\expT}
                                         & \tdExpTrans{\triple{\Multi{D}}{\fgTyEnv}{\fgEnv}}{e : \fgType}{\expT} \\
    \end{array}
  \end{mathpar}
}




==> currying.tex <==
\pagebreak
\section{Currying}

\subsection{NEW}

To fix the proof of Lemma~\ref{subtyping-equiv} (case \Rule{coerce-struct-iface}) requires a new version of
\Cref{lem:method-lookup}.

\begin{lemma}[NEW \Cref{lem:method-lookup}]
  \label{lem:new-method-lookup}
  Assume $\LREquivNoTy{\fgDecls}{k}{\tlMethTable}$ and
  $\LREquiv{\fgTySubst}{\tlSubst}{\fgTyEnv}{k}$.
  Let $ \tdMethods{R}{V}{\fgTyEnv}{t_S[\fgTyActuals]}$.
  Then there exists $U$ such that $\reduceStar{\mT{m}{t_S}\,(\tlSubst V)}{U}$ and
  $\LREquiv{\methodLookup{m}{\fgTySubst t_S[\fgTyActuals]}}{U}{\fgTySubst R}{k'}$.
  for all $k' < k$.
\end{lemma}

To prove \Cref{lem:new-method-lookup}, we need an alternative form
of \Cref{lem:method-decl-equiv-implies-dict-equiv}.

\begin{lemma}[NEW \Cref{lem:method-decl-equiv-implies-dict-equiv}]
  \label{lem:new-method-decl-equiv-implies-dict-equiv}
  Assume $\LREquivNoTy{\fgFunc}{k}{X}$.
  Then the following holds:
  \begin{mathparNarrow}
    \forall k' < k, \fgTyActuals, W \DOT \LREquiv{\fgTyActuals}{W}{\fgTyFormals}{k'}
    \implies
    \exists V \DOT \reduceStar{X\,W}{V} \wedge
    \fgMakeSubst{\fgTyFormals}{\fgTyActuals}{\fgTySubst} \wedge\\
    \LREquiv{
      \Angle{x, t_S[\fgTyActuals], \fgTySubst mM, \fgTySubst e}
    }{
      V
    }{
      \fgTySubst mM
    }{k'}
  \end{mathparNarrow}
\end{lemma}

The proof of \Cref{lem:new-method-decl-equiv-implies-dict-equiv} requires a curried form
of \Rule{equiv-method-decl} (not sure if all type substitutions are correct):

  \begin{mathpar}
    \inferrule[equiv-method-decl-curried]{
      \forall k' < k, \Multi[p]{\fgType}, \Multi[p]{W} \DOT
      \fgTySubst = \Angle{\Multi{\subst{\fgTyVar}{\fgType}}} \wedge
      \LREquiv{
        \Multi{\fgType}
      }{
        \Tuple{\Multi{W}}
      }{\Multi{\fgTyVar\,\fgType_I}}{k'} \implies\\\\
      \exists U \DOT \reduceStar{X\,\Tuple{\Multi{W}}}{U} \wedge\\\\
      (\forall \Multi[q]{\fgType'}, \Multi[q]{W'}, v, V, \Multi[n]{v}, \Multi[n]{V} \DOT
      \fgTySubst' = \Angle{\Multi{\subst{\fgTyVar'}{\fgType'}}} \wedge
      \LREquiv{
        \Multi{\fgType'}
      }{
        \Tuple{\Multi{W'}}
      }{\Multi{\fgTyVar\,\fgTySubst\fgType_I'}}{k'} \wedge\\
      \LREquiv{v}{V}{t_S[\fgTySubst \Multi{\fgTyVar}]}{k'} \wedge
      (\forall i \in [n] . \LREquiv{v_i}{V_i}{\fgTySubst\fgTySubst' \fgTypeAux_i}{k'})
      \implies\\
      \LREquiv{
        \Angle{\subst{x}{v}, \Multi{\subst{x}{v}}} \fgTySubst\fgTySubst' e
      }{
        U~V~\Tuple{\Multi{W'}}~\Tuple{\Multi{V}}
      }{
        \fgTySubst\fgTySubst' \fgTypeAux
      }{k'})
    }{
      \LREquivNoTy{\FUNC\ (x \ t_S[\Multi[p]{\fgTyVar\,\fgType_I}]) \
        m[\Multi[q]{\fgTyVar'\,\fgType_I'}](\Multi[n]{x\ \fgTypeAux})\, \fgTypeAux \
        \{ \RETURN\ e \}}{k}{X}
    }
  \end{mathpar}

  The changes to rule \Rule{equiv-method-decl} requires changes to the proof of
  \Cref{lem:method-equiv} as well changes to the proof of~\Cref{lem:exp-equiv}.

\subsection{Old}
\begin{lemma}[Old \Cref{lem:method-decl-equiv-implies-dict-equiv}]
  Assume $\LREquivNoTy{\fgFunc}{k}{X}$.
  Then the following holds:
  \begin{mathparNarrow}
    \forall k' < k, \fgTyActuals, W \DOT \LREquiv{\fgTyActuals}{W}{\fgTyFormals}{k'}
    \implies
    \fgMakeSubst{\fgTyFormals}{\fgTyActuals}{\fgTySubst} \wedge\\
    \LREquiv{
      \Angle{x, t_S[\fgTyActuals], \fgTySubst mM, \fgTySubst e}
    }{
      \tllambda{\Triple{Y_1}{Y_2}{Y_3}} X\,\Quadr{W}{Y_1}{Y_2}{Y_3}
    }{
      \fgTySubst mM
    }{k'}
  \end{mathparNarrow}
\end{lemma}

\begin{lemma}[Old \Cref{lem:method-lookup}]
  Assume $\LREquivNoTy{\fgDecls}{k}{\tlMethTable}$ and
  $\LREquiv{\fgTySubst}{\tlSubst}{\fgTyEnv}{k}$.
  Let $ \tdMethods{R}{V}{\fgTyEnv}{t_S[\fgTyActuals]}$ and
  define $U = \tllambda{\TripleY}{\mT{m}{t_S}}\,\Quadr{\tlSubst V}{Y_1}{Y_2}{Y_3}$.
  Then we have for all $k' < k$ that
  $\LREquiv{\methodLookup{m}{\fgTySubst t_S[\fgTyActuals]}}{U}{\fgTySubst R}{k'}$.
\end{lemma}

Old version of rule \Rule{equiv-method-decl}

  \begin{mathpar}
    \inferrule[equiv-method-decl]{
      \forall k' < k, \Multi[p]{\fgType}, \Multi[q]{\fgType'}, \Multi[p]{W},
      \Multi[q]{W'}, v, V, \Multi[n]{v}, \Multi[n]{V} .\\
      \fgTySubst = \Angle{\Multi{\subst{\fgTyVar}{\fgType}}, \Multi{\subst{\fgTyVar'}{\fgType'}}} \wedge
      \LREquiv{
        \Multi{\fgType} \Multi{\fgType'}
      }{
        \Tuple{\Multi{W}, \Multi{W'}}
      }{\Multi{\fgTyVar\,\fgType_I}, \Multi{\fgTyVar'\,\fgType_I'}}{k'}
      \wedge\\
      \LREquiv{v}{V}{t_S[\fgTySubst \Multi{\fgTyVar}]}{k'} \wedge
      (\forall i \in [n] . \LREquiv{v_i}{V_i}{\fgTySubst \fgTypeAux_i}{k'})
      \implies\\
      \LREquiv{
        \Angle{\subst{x}{v}, \Multi{\subst{x}{v}}} \fgTySubst e
      }{
        X~\Quadr{\Tuple{\Multi{W}}}{V}{\Tuple{\Multi{W'}}}{\Tuple{\Multi{V}}}
      }{
        \fgTySubst \fgTypeAux
      }{k'}
    }{
      \LREquivNoTy{\FUNC\ (x \ t_S[\Multi[p]{\fgTyVar\,\fgType_I}]) \
        m[\Multi[q]{\fgTyVar'\,\fgType_I'}](\Multi[n]{x\ \fgTypeAux})\, \fgTypeAux \
        \{ \RETURN\ e \}}{k}{X}
    }
  \end{mathpar}


==> translation-assertions.tex <==
\section{Dictionary-Passing Translation With Type Assertions}
\label{sec:translation-assertions}

\boxfig{f:fgg-assertions}{Syntax of FGG with type assertions}{
\bda{ll}
\ba{ll}
\GoSynCatName{Expression} & d,e ::= \ldots \mid e.(\fgType)
\ea
\eda
}

\boxfig{f:fgg-dynamic-assertions}{Dynamic semantics of FGG with type assertions}{
  \bda{llrl}
  \sSynCatName{Value} &
  v & ::= & \fgType_S \{ \ForeachN{v} \}
  \\
  \sSynCatName{Evaluation context} &
  \EvCtx & ::= & \Hole
   \mid \fgType_S \{ \ForeachN{v}, \EvCtx, \ForeachN{e} \}
   \mid \EvCtx.f
   \mid \EvCtx.(\fgType)
   \mid \EvCtx.m[\fgTyActuals](\ForeachN{e})
   \mid v.m[\fgTyActuals](\ForeachN{v}, \EvCtx, \ForeachN{e})
   \\
   \sSynCatName{Value substitution} &
   \vbFG & ::= & \LrAngle{\ForeachN{\subst{x_i}{v_i}}}
   \\
   \sSynCatName{Type substitution} &
   \tbFG & ::= & \LrAngle{\ForeachN{\subst{\fgTyVar_i}{\fgType_i}}}
   \\
   \sSynCatName{FGG type environment} & \fgTyEnv & ::= & \{ \Multi{\fgTyVar_i : {\fgType_I}_i} \}
   \eda
  \sTransSection{
    \ruleform{
      \fgMakeSubst{\fgTyFormals}{\fgTyActuals}{\fgTySubst} \qquad
      \fgCheckSubst{\fgTyEnv}{\fgTyFormals}{\fgTyActuals}{\fgTySubst}
    }
  }{Type instantiations}
  \begin{mathpar}
    \inferrule[fg-subst-unchecked]{
      \fgTyFormals = \Foreach{\fgTyVar\, \fgType}{n}
    }{
      \fgMakeSubst{\fgTyFormals}{\Foreach{\fgTypeAux}{n}}{\Angle{\Foreach{\subst{\fgTyVar_i}{\fgTypeAux_i}}{n}}}
    }

    \inferrule[fg-subst-checked]{
      \fgTyFormals = \Foreach{\fgTyVar\, \fgType}{n} \\
      \fgTySubst = \Angle{\Foreach{\subst{\fgTyVar_i}{\fgTypeAux_i}}{n}} \\
      \fgSub{\fgTyEnv}{\fgTypeAux_i}{\fgTySubst \fgType_i} \quad \noteForall{i \in [n]}
    }{
      \fgCheckSubst{\fgTyEnv}{\fgTyFormals}
        {\Foreach{\fgTypeAux}{n}}{\fgTySubst}
    }
  \end{mathpar}

  \sTransSection{
    \ruleform{\methodSpecsWithEnv{\fgTyEnv}{\fgType} = \{\Multi{R}\} }
  }{
    Method sets
  }
  \begin{mathpar}
    \inferrule[methods-struct]{}{
    \methodSpecsWithEnv{\fgTyEnv}{t_S[\fgTyActuals]} =
    \{ \fgTySubst (mM) \mid
    {\ba[t]{l}\FUNC\ (x \ t_S[\fgTyFormals]) \, mM \, \{ \RETURN\ e \} \in  \ForeachN{D},\\
    \fgCheckSubst{\fgTyEnv}{\fgTyFormals}{\fgTyActuals}{\fgTySubst} \}
    \ea}
  }

  \inferrule[methods-iface]{
    \TYPE\ t_I[\fgTyFormals] \ \INTERFACE\ \{ \ForeachN{R} \} \in \ForeachN{D}\\
    \fgMakeSubst{\fgTyFormals}{\fgTyActuals}{\fgTySubst}
  }
  { \methodSpecsWithEnv{\fgTyEnv}{t_I[\fgTyActuals]} = \{ \fgTySubst\ForeachN{R} \}
  }
  \quad
  \inferrule[methods-var]{
    (\fgTyVar : \fgType_I) \in \fgTyEnv
  }{
    \methodSpecsWithEnv{\fgTyEnv}{\fgTyVar} =
    \methodSpecsWithEnv{\fgTyEnv}{\fgType_I}
  }
  \end{mathpar}

\sTransSection{
  \ruleform{\fgSub{\fgTyEnv}{\fgType}{\fgTypeAux}}
}{Subtyping}
  \begin{mathpar}
  \inferrule[sub-refl-var]{
   }
  { \fgSub{\fgTyEnv}{\fgTyVar}{\fgTyVar}
  }

  \inferrule[sub-refl-struct]{
   }
  { \fgSub{\fgTyEnv}{\fgType_S}{\fgType_S}
  }

  \inferrule[sub-iface]{
   \methodSpecsWithEnv{\fgTyEnv}{\fgType} \supseteq \methodSpecsWithEnv{\fgTyEnv}{\fgTypeAux_I}
  }
  { \fgSub{\fgTyEnv}{\fgType}{\fgTypeAux_I}
  }
  \end{mathpar}

  \bda{llcl}
  \eda

\sTransSection{
  \ruleform{\reduce{e}{e'}}
}{
  Reductions
}
\begin{mathpar}
 \inferrule[fg-context]
 { \reduce{e}{e'}
 }
 { \reduce{\EvCtx [e]}{\EvCtx [e']}
 }

 \inferrule[fg-field]
 { \TYPE\ t_S[\fgTyFormals] \ \STRUCT\ \{ \Foreach{f \ \fgType}{n} \} \in  \ForeachN{D}\\
 }
 {  \reduce{t_S[\fgTyActuals] \{ \Foreach{v}{n} \}.f_i}{v_i}
 }

 \inferrule[fg-call]
  { v = t_S[\fgTyActuals] \{ \ForeachN{v} \}
    \\ \FUNC\ (x \ t_S[\fgTyFormals]) \ m[\fgTyFormalsAux] (\ForeachN{x \ \fgType}) \ \fgType \ \{ \RETURN\ e \} \in \ForeachN{D}
    \\ \fgMakeSubst{(\fgTyFormals, \fgTyFormalsAux)}{(\fgTyActuals, \fgTyActualsAux)}{\fgTySubst}
 }
 { \reduce{v.m[\fgTyActualsAux](\ForeachN{v})}
   {\LrAngle{\subst{x}{v}, \ForeachN{\subst{x_i}{v_i}}} \fgTySubst e}
 }

 \inferrule[fg-assert]
 { v = \fgType_S \{ \ForeachN{v} \}
   \\ \fgSub{\fgEmptyTyEnv}{\fgType_S}{\fgTypeAux}
 }
 {  \reduce{v.(\fgTypeAux)}{v}
 }
\end{mathpar}
}

\boxfig{f:target-lang-equality}{Target Language with equality}{
  \bda{lcr}
  {
    \ba{lll}
    \sSynCatName{Expression} & \expT ::=
    \\ \quad \sSynCatName{Variable}    & \quad \xT \mid \yT         & \mid
    \\ \quad \sSynCatName{Constructor} & \quad \kT                  & \mid
    \\ \quad \sSynCatName{Application} & \quad \expT \ \expT        & \mid \
    \\ \quad \sSynCatName{Abstraction} & \quad \lambda \xT. \expT   & \mid
    \\ \quad \sSynCatName{Pattern case} & \quad \tcaseof{\expT}{\ForeachN{\clsT}} & \mid
    \\ \quad \sSynCatName{Equality}    & \quad \eqT{\expT}{\expT} & \mid
    \\ \quad \sSynCatName{Error}       & \quad \ErrT
    \ea
  }
  &~\quad~&
  {
    \ba{lrl}
     \sSynCatName{Pattern clause} &
     \clsT & ::=  \patT \rightarrow \expT
     \\
     \sSynCatName{Pattern} &
     \patT & ::= \kT \ \ForeachN{\xT}
     \\
    \sSynCatName{Program}  &
    \program & ::= \LET\ \ForeachN{\yT_i = V_i} \ \IN\ \expT
    \ea
   }
   \eda
  \bda{l@{\quad}lrl}
  \sSynCatName{TL values} &
  \uT & ::= & \kT\ \ForeachN{\uT} \mid \lambda \xT . \expT
  \\
  \sSynCatName{TL evaluation context} &
  \REvCtxT & ::= & \Hole
   \mid \tcaseof{\REvCtxT}{\Multi{\clsT}}
   \mid \REvCtxT\ \expT
   \mid \uT\ \REvCtxT
   \\ && \mid & \eqT{\REvCtxT}{\expT}
   \mid \eqT{\valT}{\REvCtxT}
  \\
     \sSynCatName{TL substitution} &
   \vbTL, \vbMethTL & ::= & \Angle{\ForeachN{\subst{\xT}{\uT}}}
   \eda
\vspace{1ex}
\sTransSection{
  \ruleform{
    \reduceExpTL{\vbMethTL}{\expT}{\expT'}
  }
}{
  TL expression reductions
}
\vspace{-0.5ex}
\begin{mathpar}
 \inferrule[tl-context]
 {\reduceExpTL{\vbMethTL}{\expT}{\expT'}
 }
 {\reduceExpTL{\vbMethTL}{\REvCtxT [\expT]}{\REvCtxT [\expT']}
 }

 \inferrule[tl-lambda]
 {}
 { \reduceExpTL{\vbMethTL}{(\lambda \xT. \expT) \ \uT}{\Angle{\subst{\xT}{\uT}} \expT}
 }

 \inferrule[tl-case]
 { \kT \ \Multi{\xT} \rightarrow \expT \in \Multi{\clsT}
 }
 {\reduceExpTL{\vbMethTL}{\tcaseof{\kT \ \Multi{\uT}}{\Multi{\clsT}}}
         {\Angle{\Multi{\subst{\xT_i}{\uT_i}}} \expT}
 }

 \inferrule[tl-method]{}{
   \reduceExpTL{\vbMethTL}{\xT}{\vbMethTL(\xT)}
 }

 \inferrule[tl-eq]{
   \kT = {
     \begin{cases}
       \trueT & \textrm{if}~ \valT = \valT'\\
       \falseT & \textrm{otherwise}
     \end{cases}
   }
 }{
   \reduceExpTL{\vbMethTL}{\eqT{\valT}{\valT'}}{\kT}
 }

\end{mathpar}

\vspace{1ex}
\sTransSection{
  \ruleform{\reduceTL{\program}{\program'}}
}{
  TL reductions
}
\vspace{-0.5ex}
\begin{mathpar}
  \inferrule[tl-prog]{
    \vbMethTL = \Angle{\ForeachN{\subst{\yT_i}{V_i}}}\\
    \reduceExpTL{\vbMethTL}{\expT}{\expT'}
  }{
    \reduceTL{\tletrecin{\ForeachN{\yT_i = V_i}}{\expT}}{\tletrecin{\ForeachN{\yT_i = V_i}}{\expT'}}
  }
\end{mathpar}
} %

\subsection{Translating programs, methods and expressions}

\boxfig{f:value-repr-assertions}{Representations of FGG values}{
  \begin{itemize}
  \item A dictionary $\mathcal D$ for method signatures $\Foreach{M}{n}$ is an $n$-element list
    $\List{\Foreach{E}{n}}$,
    where $E_i$ is evidence for an implementation of a method with signature $M_i$.
  \item A type variable $\fgTyVar$
    is represented as $\Tuple{E_1\Comma E_2\Comma E_3}$, where $E_1$ is the nominal representation of
    the type substituted for $\fgTyVar$, $E_2$ is the structural representation of this type and $E_3$ is a function taking
    a value of this type to the bound of $\fgTyVar$.
  \item A value of type $\fgType_S$ is represented as $\Tuple{E\Comma \Tuple{\ForeachN{E'}}}$ where $E$ is the nominal representation
    of the type $\fgType_S$ and $E_i'$ is the value of the $i$-th field of the struct.
  \item A value of type $\fgType_I$ is represented as an interface value $\Tuple{E\Comma E'\Comma \mathcal D}$ where $E$ is a list
    representing the method specifications of $\fgType_I$,
    $E'$ is the concrete value hidden behind the interface type, and $\mathcal D$
    is the dictionary for the methods of the interface.
  \end{itemize}
}

\boxfig{f:fgg-type-ok-assertions}{Wellformedness of FGG types}{
  FIXME: defined as in the FGG paper
  \begin{mathpar}
    \fgTyOk{\fgTyEnv}{\fgType}\quad
    \fgTyOk{\fgTyEnv}{\ForeachN{\fgType}}\quad
    \fgOk{\fgTyFormals; \fgTyFormalsAux}\,\fgTyEnv\quad
    \subtypeOf{\fgTyFormals}{\fgTyFormals'}\quad
    \fgOk{\TYPE\ t[\fgTyFormals]\,L}
  \end{mathpar}
}
\boxfig{f:trans-defs-assertions}{Conventions and definitions for the translation}{
  Convention for mapping to target terms
  \vspace{-1ex}
  \begin{mathpar}
    x \leadsto \xT
    \quad
    \fgTyVar \leadsto \xTyt{\fgTyVar}, \xTys{\fgTyVar}, \xTyb{\fgTyVar}
    \quad
    t_S \leadsto K_{t_S}
    \quad
    t_I \leadsto K_{t_I}
    \quad
    m \leadsto K_{m}
    \\
    \textrm{natural number {\bf i} (De Bruijn index)} \leadsto \DeBruijnIndex{i}
    \qquad
    \FUNC\ (x \ {t_S}[\fgTyFormals]) \, m M \, \{ \RETURN\ e \} \leadsto \mT{m}{t_S}
  \end{mathpar}

  \bda{llcl}
  \mbox{FGG value environment}  & \fgEnv      & ::= & \{ \ForeachN{x : \fgType} \}\\
  \mbox{Type-expression environment} & \tdTyVarEnv & ::= & \{ \ForeachN{\fgTyVar : E} \}
  \eda
  \vspace{0.5ex}
}

\boxfig{f:trans-types-assertions}{Translation of types and method specifications}{
  \sTransSection{
    \ruleform{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgType}{E} \qquad
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\ForeachN{\fgType}}{E} \qquad
      \tdTypeTrans{\fgTyEnv}{\fgType}{E}
    }
  }{
    Translating types
  }
  \begin{mathpar}
    \inferrule[tyvar-var]{
      \fgTyVar \notin \tdTyVarEnv\\
      (\fgTyVar : \fgType) \in \fgTyEnv
    }{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgTyVar}{\xTyt{\fgTyVar}}
    }

    \inferrule[tyvar-exp]{
      \fgTyVar \notin \fgTyEnv\\
      (\fgTyVar : E) \in \tdTyVarEnv
    }{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgTyVar}{E}
    }

    \inferrule[named-type]{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgTyActuals}{E}
    }{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{t[\fgTyActuals]}{K_t\,E}
    }

    \inferrule[types]{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgType_i}{E_i} \quad \noteForall{i \in [n]}
    }{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\Foreach{\fgType}{n}}{\Tuple{\Foreach{E}{n}}}
    }

    \inferrule[type]{
      \tdTypeTrans{\pair{\fgTyEnv}{\fgEmptyEnv}}{\fgType}{E}
    }{
      \tdTypeTrans{\fgTyEnv}{\fgType}{E}
    }
  \end{mathpar}

  \sTransSection{
    \ruleform{
      \tdSigTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{M}{E}\quad
      \tdSpecTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{R}{E}
    }
  }{
    Translating method specifications
  }
  \begin{mathpar}
    \inferrule[sig]{
      \fgTyFormals = \Foreach{\fgTyVar\, \fgTypeAux}{q}\\
      \tdTyVarEnv' = \tdTyVarEnv \cup \{ \Foreach{ \fgTyVar_i : \DeBruijnIndex{i} }{q} \}\\
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv'}}{\Foreach{\fgTypeAux}{q}}{E}\\
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv'}}{\Foreach{\fgType}{n} \fgType}{E'}
    }{
      \tdSigTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{[\fgTyFormals](\Foreach{x~\fgType}{n})\,\fgType}{\Tuple{E\Comma E'}}
    }

    \inferrule[spec]{
      \tdSigTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{M}{E}
    }{
      \tdSpecTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{mM}{K_m\,E}
    }
  \end{mathpar}

  \sTransSection{
    \ruleform{
      \tdTypeStarTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgType}{E}\quad
      \tdTypeStarTrans{\fgTyEnv}{\fgType}{E}
    }
  }{
    Translating runtime types
  }
  \begin{mathpar}
    \inferrule[tyvar*]{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgTyVar}{E}
    }{
      \tdTypeStarTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgTyVar}{E}
    }

    \inferrule[struct*]{
      \tdTypeTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgType_S}{E}
    }{
      \tdTypeStarTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgType_S}{E}
    }

    \inferrule[iface*]{
      \TYPE\ t[\fgTyFormals]\ \INTERFACE\ \{ \Foreach{R}{n} \} \in \fgDecls\\
      \fgMakeSubst{\fgTyFormals}{\fgTyActuals}{\fgTySubst}\\
      \tdSpecTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{\fgTySubst R_i}{E_i}\quad\noteForall{i \in [n]}
    }{
      \tdTypeStarTrans{\pair{\fgTyEnv}{\tdTyVarEnv}}{t_I[\fgTyActuals]}{\List{\Foreach{E}{n}}}
    }

    \inferrule[type*]{
      \tdTypeStarTrans{\pair{\fgTyEnv}{\fgEmptyEnv}}{\fgType}{E}
    }{
      \tdTypeStarTrans{\fgTyEnv}{\fgType}{E}
    }
  \end{mathpar}

} %

\boxfig{f:trans-auxiliaries-assertions}{Auxiliaries for translation}{
  \sTransSection{
    \ruleform{
      \tdCheckSubst{\fgTyEnv}{\fgTyFormals}{\fgTyActuals}{\fgTySubst}{E}
    }
  }{Type instantiations}
  \begin{mathpar}
    \inferrule[type-inst]{
      \fgTyFormals = \Foreach{\fgTyVar\, \fgType}{n} \\
      \fgTySubst = \LrAngle{\Foreach{\subst{\fgTyVar_i}{\fgTypeAux_i}}{n}} \\
      \tdTypeTrans{\fgTyEnv}{\fgTypeAux_i}{E_i} \\
      \tdTypeStarTrans{\fgTyEnv}{\fgTypeAux_i}{E_i'} \\
      \tdUpcast{\fgTyEnv}{\subtypeOf{\fgTypeAux_i}{\fgTySubst \fgType_i}}{E_i''} \\
      \noteForall{i \in [n]}
    }{
      \tdCheckSubst{\fgTyEnv}{\fgTyFormals}
        {\Foreach{\fgTypeAux}{n}}{\fgTySubst}{\Tuple{\Multi[n]{\Triple{E_i}{E_i'}{E_i''}}}}
    }
  \end{mathpar}

  \sTransSection{
    \ruleform{\tdMethods{R}{E}{\fgTyEnv}{\fgType_S}}
  }{
    Method access
  }

  \begin{mathpar}
    \inferrule[methods-struct]{
      \FUNC\ (x \ {t_S}[\fgTyFormals]) \, m M \, \{ \RETURN\ e \} \in \fgDecls\\
      \tdCheckSubst{\fgTyEnv}{\fgTyFormals}{\fgTyActuals}{\fgTySubst}{E}\\
      R = \fgTySubst (mM)
    }{
      \tdMethods{R}{E}{\fgTyEnv}{t_S[\fgTyActuals]}
    }
  \end{mathpar}
}


\boxfig{f:trans-exp1-assertions}{Translation of expressions}{
  \sTransSection{
    \ruleform{\tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e : \fgType}{\expT}}
  }{
    Translating expressions
  }
  \begin{mathpar}
    \inferrule[var]{
      (x : \fgType) \in \fgEnv
    }{
      \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{x : \fgType}{\xT}
    }

    \inferrule[struct]{
      \fgTyOk{\fgTyEnv}{t_S[\fgTyActuals]}\\
      \TYPE\ t_S[\fgTyFormals] \ \STRUCT\ \{ \Foreach{f \ \fgType}{n} \} \in  \ForeachN{D}\\
      \tdTypeTrans{\fgTyEnv}{t_S[\fgTyActuals]}{E}\\
      \fgMakeSubst{\fgTyFormals}{\fgTyActuals}{\fgTySubst}\\
      \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e_i : \fgTySubst\fgType_i}{\expT_i}
      \quad\noteForall{i \in [n]}
    }{
      \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}
      {t_S[\fgTyActuals] \{ \Foreach{e}{n} \} : t_S[\fgTyActuals] }{\Tuple{E\Comma \Tuple{\Foreach{\expT}{n}}}}
    }

  \inferrule[access]{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e : t_S[\fgTyActuals]}{\expT} \\
    \TYPE\ t_S[\fgTyFormals] \ \STRUCT\ \{ \Foreach{f \ \fgType}{n} \} \in  \ForeachN{D}\\
      \fgMakeSubst{\fgTyFormals}{\fgTyActuals}{\fgTySubst}\\
  }{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}
    {e.f_i : \fgTySubst \fgType_i }
    { \CASE\ \expT\ \OF\ \Tuple{\wildcard\Comma \Tuple{\Foreach{\xT}{n}}} \rightarrow \xT_i}
  }

  \inferrule[call-struct]{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e : t_S[\fgTyActuals]}{\expT} \\
    \tdMethods{m[\fgTyFormalsAux](\Foreach{x\,\fgTypeAux}{n})\fgTypeAux}{E'}{\fgTyEnv}{t_S[\fgTyActuals]}\\
    \tdCheckSubst{\fgTyEnv}{\fgTyFormalsAux}{\fgTyActualsAux}{\fgTySubst}{E''}\\
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e_i: \fgTySubst \fgTypeAux_i}{\expT_i}
    \quad\noteForall{i \in [n]}
  }{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e.m[\fgTyActualsAux](\Foreach{e}{n}) : \fgTySubst \fgTypeAux}
    {\mT{m}{t_S} \ \Quadr{\expT'}{\expT}{\expT''}{\Tuple{\Foreach{\expT}{n}}} }
  }

  \inferrule[call-iface]{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e : \fgType_I}{\expT}\\
    \methodSpecsWithEnv{\fgTyEnv}{\fgType_I} = \Foreach{R}{q}\\
    R_j = m[\fgTyFormalsAux](\Foreach{x\,\fgTypeAux}{n})\fgTypeAux \quad(\textrm{for some}~j \in [q])\\
    \tdCheckSubst{\fgTyEnv}{\fgTyFormalsAux}{\fgTyActualsAux}{\fgTySubst}{E'}\\
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e_i : \fgTySubst \fgTypeAux_i}{\expT_i}
    \quad\noteForall{i \in [n]}\\
    Y, \Foreach{X}{q}\textrm{~fresh}
  }{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}
    {e.m[\fgTyActualsAux](\Foreach{e}{n}) : \fgTySubst\fgTypeAux}
    {\CASE\ \expT \ \OF\ \Tuple{\wildcard\Comma Y\Comma \List{\Foreach{X}{q}}} \to X_j\ \Triple{Y}{E'}{\Tuple{\Foreach{E}{n}}}}
  }

  \inferrule[assert]{
    \fgTyOk{\fgTyEnv}{\fgTypeAux}\\
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e : \fgType}{\expT}\\
    \tdDowncast{\fgTyEnv}{\assertOf{\fgType}{\fgTypeAux}}{V}
  }{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e.(\fgTypeAux) : \fgTypeAux}{V \ \expT}
  }

  \inferrule[sub]{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e : \fgType}{\expT}\\
    \tdUpcast{\fgTyEnv}{\subtypeOf{\fgType}{\fgTypeAux}}{V}
  }{
    \tdExpTrans{\pair{\fgTyEnv}{\fgEnv}}{e : \fgTypeAux}{V \ \expT}
  }
\end{mathpar}


}


\boxfig{f:upcast-assertions}{Translation of structural subtyping}{

  \sTransSection{
  \ruleform{\tdUpcast{\fgTyEnv}{\subtypeOf{\fgType}{\fgTypeAux}}{V}}
}{
  Interface-value construction
}
\begin{mathpar}
  \inferrule[coerce-tyvar]{
    X~\textrm{fresh}\\
    (\fgTyVar : \fgTypeAux_I) \in \fgTyEnv\\
    \tdUpcast{\fgTyEnv}{\subtypeOf{\fgTypeAux_I}{\fgType}}{V}
  }{
    \tdUpcast{\fgTyEnv}{\subtypeOf{\fgTyVar}{\fgType}}
      {\tllambda{X} V\, (\xTyb{\fgTyVar}\, X)}
  }

  \inferrule[coerce-struct-iface]{
    X, Y_1, Y_2, Y_3~\textrm{fresh}\\
    \TYPE\ t_I[\fgTyFormals] \ \INTERFACE\ \{ \Foreach{mM}{n} \} \in \ForeachN{D}\\
    \tdTypeStarTrans{\fgTyEnv}{t_I[\fgTyActuals]}{E}\\
    \fgMakeSubst{\fgTyFormals}{\fgTyActuals}{\fgTySubst}\\
    \tdMethods{\fgTySubst(m_i M_i)}{E_i}{\fgTyEnv}{t_S[\fgTyActualsAux]}\\
    E_i' = \PartialM{\mT{m_i}{t_S}}{E_i}
    \quad\noteForall{i \in [n]}
  }{
    \tdUpcast{\fgTyEnv}{\subtypeOf{t_S[\fgTyActualsAux]}{t_I[\fgTyActuals]}}
    {\tllambda{\xT} \Tuple{E\Comma \xT\Comma \List{\Foreach{E_i'}{n}}} }
  }

  \inferrule[coerce-iface-iface]{
    Y,\Foreach{X}{n}~\textrm{fresh}\\
    \mapPerm : [q] \to [n]~\textrm{total}\\
    \TYPE\ t_I[\fgTyFormals_1] \ \INTERFACE\ \{ \Foreach{R}{n} \} \in \ForeachN{D}  \\
    \TYPE\ u_I[\fgTyFormals_2] \ \INTERFACE\ \{ \Foreach{R'}{q} \} \in \ForeachN{D}  \\
    \tdTypeStarTrans{\fgTyEnv}{u_I[\fgTyActuals_2]}{E}\\
    \fgMakeSubst{\fgTyFormals_1}{\fgTyActuals_1}{\fgTySubst_1}\\
    \fgMakeSubst{\fgTyFormals_2}{\fgTyActuals_2}{\fgTySubst_2}\\
    \fgTySubst_2 R'_i = \fgTySubst_1 R_{\mapPerm(i)} \quad\noteForall{i \in [q]}
  }{
    \tdUpcast{\fgTyEnv}{\subtypeOf{t_I[\fgTyActuals_1]}{u_I[\fgTyActuals_2]}}
    { \tllambda{\Tuple{\wildcard\Comma Y\Comma \List{\Foreach{X}{n}}}}
      \Tuple{E\Comma Y\Comma \List{\xT_{\mapPerm(1)}\Comma \ldots\Comma \xT_{\mapPerm(q)}}}
    }
  }
\end{mathpar}
}%

\boxfig{f:downcast-assertions}{Translation of type assertions}{
\sTransSection{
  \ruleform{\tdDowncast{\fgTyEnv}{\assertOf{\fgType}{\fgTypeAux}}{V}}
}{
  Interface-value destruction
}
\begin{mathpar}
  \inferrule[destr-struct-struct]{
    Y~\textrm{fresh}\\
    \tdTypeTrans{\fgTyEnv}{\fgTypeAux_S}{E}
  }{
    \tdDowncast{\fgTyEnv}{\assertOf{\fgType_S}{\fgTypeAux_S}}
    {\tllambda{Y}
      \CASE\ \eqT{\expT}{\fst\, Y}\ \OF\ \trueT \to Y, \falseT \to \ErrT
    }
  }

  \inferrule[destr-iface-struct]{
    Y~\textrm{fresh}\\
    \tdTypeTrans{\fgTyEnv}{\fgTypeAux_S}{E}
  }{
    \tdDowncast{\fgTyEnv}{\assertOf{\fgType_I}{\fgTypeAux_S}}
    {\tllambda{\Tuple{\wildcard\Comma Y\Comma \wildcard}}
      \CASE\ \eqT{\expT}{\fst\, Y}\ \OF\ \trueT \to Y, \falseT \to \ErrT
    }
  }

  \inferrule[destr-struct-iface]{
    Y~\textrm{fresh}\\
    \tdTypeStarTrans{\fgTyEnv}{\fgTypeAux_I}{E}\\
  }{
    \tdDowncast{\fgTyEnv}{\assertOf{\fgType_S}{\fgTypeAux_I}}
    {\tllambda{Y} \dynAssert{Y}{E}}
  }

  \inferrule[destr-iface-iface]{
    Y~\textrm{fresh}\\
    \tdTypeStarTrans{\fgTyEnv}{\fgTypeAux_I}{E}\\
  }{
    \tdDowncast{\fgTyEnv}{\assertOf{\fgType_I}{\fgTypeAux_I}}
    {\tllambda{\Tuple{\wildcard\Comma Y\Comma \wildcard}} \dynAssert{Y}{E}}
  }

  \inferrule[destr-struct-tyvar]{
    Y~\textrm{fresh}\\
    \fgTyVar \in \domT(\fgTyEnv)
  }{
    \tdDowncast{\fgTyEnv}{\assertOf{\fgType_S}{\fgTyVar}}
    {\tllambda{Y}
      \ba[t]{l}
      \CASE\ \eqT{\xTyt{\fgTyVar}}{\fst\, Y}\ \OF\\
      \quad \trueT \to Y\\
      \quad \falseT \to \dynAssert{Y}{\xTys{\fgTyVar}}
      \ea
    }
  }

  \inferrule[destr-iface-tyvar]{
    Y~\textrm{fresh}\\
    \fgTyVar \in \domT(\fgTyEnv)
  }{
    \tdDowncast{\fgTyEnv}{\assertOf{\fgType_I}{\fgTyVar}}
    {\tllambda{\Tuple{\wildcard\Comma Y\Comma \wildcard}}
      \ba[t]{l}
      \CASE\ \eqT{\xTyt{\fgTyVar}}{\fst\, Y}\ \OF\\
      \quad \trueT \to Y\\
      \quad \falseT \to \dynAssert{Y}{\xTys{\fgTyVar}}
      \ea
    }
  }

  \inferrule[destr-tyvar]{
    X~\textrm{fresh}\\
    (a : \fgTypeAux_I) \in \fgTyEnv\\
    \tdDowncast{\fgTyEnv}{\assertOf{\fgTypeAux_I}{\fgType}}{V}
  }{
    \tdDowncast{\fgTyEnv}{\assertOf{\fgTyVar}{\fgType}}
    {\tllambda{X} V\,(\xTyb{\fgTyVar}\,X)}
  }
\end{mathpar}
} %

\boxfig{f:trans-meth-prog-assertions}{Translation of methods and programs}{
\sTransSection{
  \ruleform{\tdMethTrans{\FUNC\ (x \ t_S[\fgTyFormals])\,R\,\{\RETURN\,e\}}{X = \expT} }
}{
  Translating method declarations
}
\begin{mathpar}
  \inferrule[method]{
    \ForeachN{D}~\textrm{does not contain another}~\FUNC~\textrm{declaration for}~t_S, m\\
    \distinct{x,\Foreach{x}{n}}\\
    (\TYPE\ t_S[\fgTyFormals']\,L) \in \fgDecls\\
    \subtypeOf{\fgTyFormals}{\fgTyFormals'}\\
    \fgOk{\fgTyFormals; \fgTyFormalsAux}\,\fgTyEnv\\
    \fgTyOk{\fgTyEnv}{\Foreach{\fgType}{n}\,\fgType}\\
    \fgGetTyVars{\fgTyFormals} = \Foreach{\fgTyVar}{q}\\
    \fgGetTyVars{\fgTyFormalsAux} = \Foreach{\fgTyVarAux}{k}\\
    \tdExpTrans
      {\pair{\fgTyEnv}{\{ x : t_S[\Foreach{\fgTyVar}{q}], \Foreach{x_i : \fgType_i}{n} \}}}
      {\hasTypeSub{e}{\fgType}}{\expT}
      \\
      E' = \lambda \Quadr{\Tuple{\Multi[q]{\Triple{\xTyt{\fgTyVar_i}}{\xTys{\fgTyVar_i}}{\xTyb{\fgTyVar_i}}}}}
                         {X}
                         {\Tuple{\Multi[k]{\Triple{\xTyt{\fgTyVarAux_i}}{\xTys{\fgTyVarAux_i}}{\xTyb{\fgTyVarAux_i}}}}}
                         {\Tuple{\Multi[n]{X}}}
           . E
  }{
    \tdMethTrans
    {\FUNC\ (x \ t_S[\fgTyFormals]) \,
      m[\fgTyFormalsAux](\Foreach{x \ \fgType}{n}) \ \fgType \ \{ \RETURN\ e \}}
    {\mT{m}{t_S} = \expT'}
  }
\end{mathpar}

\sTransSection{
  \ruleform{\tdImplClause{\FUNC\ (x \ t_S[\fgTyFormals])\,R}{\clsT}
  }
}{
  Checking method implementation
}
\begin{mathpar}
  \inferrule[method-impl]{
    \fgTyFormals = \Foreach{\fgTyVar\,\fgType}{n}\\
    X, Y, \Foreach{X}{n}, \Multi[3]{Y}~\textrm{fresh}\\
    \tdTyVarEnv = \{ \Foreach{\fgTyVar_i : X_i}{n} \}\\
    \tdSigTrans{\pair{\fgEmptyEnv}{\tdTyVarEnv}}{M}{E}\\
    \tdTypeStarTrans{\pair{\EmptyFgTyEnv}{\tdTyVarEnv}}{\fgType_i}{E_i'}\\
    E_i = \Triple{X_i}{\starTy\ X_i}{\tllambda{Y} \dynAssert{\unpack\,Y}{E_i'}}
    \quad\noteForall{i \in [n]} \\
    E' = \PartialM{\mT{m_i}{t_S}}{\Tuple{\Multi[n]{E}}}
  }{
    \tdImplClause{\FUNC\ (x \ t_S[\fgTyFormals])\, mM}{
      {\ba[t]{l}
      (K_{t_S}(\Foreach{X}{n}), K_m\,X) \to\\
      \quad \CASE\ \eqT{E}{X}\ \OF\ \trueT \to E', \falseT \to \ErrT
      \ea}
    }
  }
\end{mathpar}

\sTransSection{
  \ruleform{\tdTyStarClause{\TYPE\ t[\fgTyFormals]\ L}{\clsT}}
}{
  Runtime translation of types
}
\begin{mathpar}
  \inferrule[star-ty]{
    \Multi[n]{X}~\textrm{fresh}\\
    \tdTyVarEnv = \{ \Foreach{\fgTyVar_i : X_i}{n} \}\\
    \tdTypeStarTrans{\pair{\EmptyFgTyEnv}{\tdTyVarEnv}}{t[\Multi[n]{\fgTyVar}]}{E}
  }{
    \tdTyStarClause{
      \TYPE\ t[\Multi[n]{\fgTyVar\,\fgType}] \ L
    }{
      K_t(\Multi[n]{X}) \to E
    }
  }
\end{mathpar}

\sTransSection{
  \ruleform{\tdProgTrans{P}{\program}}
}{
  Translating programs
}
\begin{mathpar}
  \inferrule[prog]{
    X~\textrm{fresh}\\
    \tdExpTrans{\pair{\EmptyFgEnv}{\EmptyFgEnv}}{e : \fgType}{\expT} \\
    \fgDeclOk{D_i} \\
    \tdTyStarClause{D_i}{\clsT_i}\\
    (\textrm{for all}~D_i \in \ForeachN{D} ~\textrm{with}~D_i = \TYPE\,\ldots)\\\\
    \tdMethTrans{D_i'}{X_i = \expT_i}\\
    \tdImplClause{D_i'}{\clsT'_i}\quad
    (\textrm{for all}~D_i' \in \ForeachN{D} ~\textrm{with}~ D_i' = \FUNC\,\ldots)\\
 }
 { \TurnsTdProg
   { \ba[t]{l}
     {\ForeachN{D} \ \FUNC\ \MAIN () \{ \_ = e \}} \leadsto \\
     \LET\
       \ba[t]{ll}
       \fst &= \tllambda{\Tuple{X\Comma \wildcard}} X\\
       \snd &= \tllambda{\Tuple{\wildcard\Comma X}} X\\
       \tyStar &= \tllambda{X} \CASE\ X\ \OF\ \ForeachN{\clsT}\\
       \unpack &= \tllambda{X} \CASE\, X\, \OF\, \Triple{\wildcard}{Y}{\wildcard} \to Y, \wildcard \to X \\
       \impl &= \tllambda{X} \CASE\ X\ \OF\ \ForeachN{\clsT'}, \wildcard \to \ErrT\\
       \getDict &= \tllambda{\Tuple{\textit{Ty}\Comma \textit{Sigs}}} \CASE\ \textit{Sigs}\ \OF\\
       &\qquad \List{} \to \List{} \\
       &\qquad \Cons{X}{\textit{Xs}} \to \Cons{\impl\,\Tuple{\textit{Ty}\Comma X}}{\getDict\,\Tuple{\textit{Ty}\Comma \textit{Xs}}}\\
       \dynAssertName &= \tllambda{\Tuple{\textit{Val}\Comma \textit{Sigs}}}
         \Tuple{\textit{Sigs}\Comma \textit{Val}\Comma \getDict\,\Tuple{\fst\,\textit{Val}\Comma \textit{Sigs}}}\\
       \ForeachN{X_i = \expT_i}
       \ea
     \\
     \IN\ \expT
     \ea
   }
 }
\end{mathpar}
} %

Additional well-formedness conditions:
\begin{description}
\item[\FGGStructNonRec:] Structs must be non-recursive. (Not checked by FGG)
\item[\FGGUniqueFields:] For each struct, field names must be distinct. (Checked with $\fgDeclOk{\cdot}$)
\item[\FGGUniqueMethSpec:] For each interface, method names must be distinct. (Checked with $\fgDeclOk{\cdot}$)
\item[\FGGUniqueReceiver:] Each method definition is uniquely identified by the receiver type and method name.
  (Checked in \RefTirName{method})
\end{description}




==> translation-output.tex <==
\section{Formal Translation Applied to Examples}
\label{sec:form-transl-appl}


